Greener yet Powerful: Taming Large Code Generation Models with Quantization

ML-powered code generation aims to assist developers to write code in a more productive manner, by intelligently generating code blocks based on natural language prompts. Recently, large pretrained deep learning models have substantially pushed the boundary of code generation and achieved impressive performance. Despite their great power, the huge number of model parameters poses a significant threat to adapting them in a regular software development environment, where a developer might use a standard laptop or mid-size server to develop her code. Such large models incur significant resource usage (in terms of memory, latency, and dollars) as well as carbon footprint. Model compression is a promising approach to address these challenges. Several techniques are proposed to compress large pretrained models typically used for vision or textual data. Out of many available compression techniques, we identified that quantization is mostly applicable for code generation task as it does not require significant retraining cost. As quantization represents model parameters with lower-bit integer (e.g., int8), the model size and runtime latency would both benefit from such int representation. We extensively study the impact of quantized model on code generation tasks across different dimension: (i) resource usage and carbon footprint, (ii) accuracy, and (iii) robustness. To this end, through systematic experiments we find a recipe of quantization technique that could run even a $6$B model in a regular laptop without significant accuracy or robustness degradation. We further found the recipe is readily applicable to code summarization task as well.

==> 5_related.tex <==
\section{Related Work}


%\subsection{Pretrained Model for Code Intelligence}


%Pretrained Language Models (PLMs) have become the predominant paradigm for a wide variety of NLP applications such as text generation. Based on the model architecture, these PLMs can be categorized into three types: encoder-only, decoder-only and encoder-decoder models, and the latter two are typically well suited for generation tasks. 

%Inspired by the overwhelming success of pretraining paradigm on natural language tasks, applying pretraining to code-related scenarios has attracted great attention recently. CodeBERT \cite{FengZ2020} which performs pretraining Masked Language Modeling (MLM) which is shown to be effective in code search and code summarization tasks. PLBART \cite{AhmadW2021}, as a BART-based \cite{LewisM2020} encoder-decoder model, could perform both code understanding and generations tasks. Codex \cite{ChenM2021}, CodeGen \cite{NijkampE2022}, Code-T$5$ \cite{WangY2021} and Incoder \cite{FriedD2022} develop decoder-only model or encoder-decoder model for code generation, and demonstrate their effectiveness on generating functional code from NL description. Notably, AlphaCode \cite{LiY2022} further develop a pretrained model that could solve competitive programming problems by overgeneration-and-reranking, and it performs better than nearly half of participants in programming competitions on {\it Codeforces} \footnote{https://codeforces.com/} platform.


% could take into account both left and right context for performing code infilling task by using  causal masking objective \cite{AghajanyanA2022} in pretraining.

%  In particular, for text generation, pretrained language .


%GraphCodeBERT\cite{GuoD2021} , TreeGen \cite{SunZ2020a} incorporates the AST structure into pretraining.

 % \cite{WanY2022} analyzes the CodeBERT and GraphCodeBERT


%\subsection{Model Compression for Pretrained Model}

As the pretrained models become increasingly large, how to effectively compress transformer-based models has become more and more important. Models after compression would have smaller storage cost/memory usage, lower inference latency, and less consumption of computational resource (hence less carbon footprint). 

\subsection{Knowledge Distillation} Knowledge Distillation (KD) \cite{KimY2016} \cite{WangF2021} \cite{LiA2020} \cite{LiL2021} aims to transfer the knowledge from a large model (as teacher) to a relatively small student model while maintaining similar accuracy. Most existing works focus on  Notably, \cite{KimY2016} proposes and compares the performance of word-level distillation (Word-KD) and sequence-level distillation (Seq-KD) for sequence generation models.  \cite{XiaM2022} and \cite{LagunasF2021} perform joint pruning and distillation which leads to improved performance.  The downside of knowledge distillation is twofold. First, it requires storing a large teacher model in the memory during the joint training and distillation phase. Second, it typically requires training over the original large dataset which leads to significant computational cost and carbon footprint.
%ImitKD \cite{LiA2020} develops an imitation learning based approach for distilling autoregressive models which achieves promising results on text summarization and translation tasks. 
%Dynamic KD \cite{LiL2021} performs distillation with dynamic teacher and data selection and also adjusts supervision objectives when training student models. 

\subsection{Quantization} %As sequence generation is a relatively more challenging task than classification, few  studies quantizing generation model 
%I-BERT \cite{KimS2021} extends integer operation beyond matrix multiplication to other operators (e.g., sigmoid) to avoid back-and-forth quantize/dequantize operations to further speed up model inference.
Few existing works study how to effectively quantize generation model until recently. QuantGPT \cite{TaoC2022} and DQ-BART \cite{LiZ2022} develop a joint Quantization-Aware-Training (QAT) and distillation approach for quantizing GPT2 model and BART model, respectively, and they achieved promising results on text generation tasks (e.g., summarization). One concurrent work \cite{YaoZ2022} of ours studies Post Training Quantization (PTQ) for natural language generation, which achieves comparable accuracy and up to $5.2x$ speed-up compared to \texttt{fp16}. 

%Commodity hardware typically supports GEMM (General Matrix Multiply) in \texttt{int8}, recently certain type of hardware start to support \texttt{int4} computation (e.g., Nvidia Turing TensorCore).  


\subsection{Pruning} Pruning techniques can be roughly categorized into unstructured pruning \cite{GordonM2020} \cite{SanhV2020} and structured pruning \cite{VoitaE2019} \cite{SajjadH2020} \cite{McCarleyC2019} \cite{XiaM2022}. Unstructured pruning on pretrained models could prune any entry in parameter matrix without hurting the accuracy. However, there would not be much improvement in latency given the unstructured sparsity is not hardware-friendly. Structured pruning aims at prune certain modules/components, such as attention head pruning \cite{VoitaE2019}, layer pruning \cite{SajjadH2020}, FFN pruning \cite{XiaM2022}, intermediate dimension pruning \cite{McCarleyC2019} and block pruning \cite{LagunasF2021}. Both structured and unstructured pruning require training the model with sparsity constraint/regularization on the whole training data, and it is therefore computationally expensive. 

Note that most techniques above would require \zijian{partial sentence?}. Also, almost all existing works on compressing pretrained models focus on text/natural language models, how to effectively compress code generation models, however, has not been explored. To our best knowledge, our work is the first attempt on compressing state-of-the-art large pretrained models for program synthesis. 

==> case_study.tex <==
\section{Qualitative Analysis of Quantization}%  Code Generation Models}
\label{section:quantization_analysis}

In the experiments we quantitatively observe that dynamic (per-tensor) quantization tends to outperform static (per-tensor) quantization. While, static (per-column) quantization outperform static (per-tensor quantization). In this section we will qualitatively explain the reasons for these observation.

\rayb{We need a prelude here explaining what we are doing?}


% \rayb{Probably have to move this para at a later section}
% We analyze both publicly available models and in-house trained models with various sizes and architectures. 


% \begin{table}
% \begin{center}
% \caption{Model details under investigation.}
% \label{table:model_to_study}
% % \begin{tabular}{ l| c| c| c} 
% \resizebox{\linewidth}{!}{%
% \setlength{\tabcolsep}{2pt}
% \begin{tabular}{p{2cm} p{2.5cm} p{2cm} p{1.5cm}}
% \toprule
%  Models & \#Parameters & Training Steps & Architecture  \\ \midrule
% PLBART  & 140M (base) & 100k & Enc-Dec \\  %\hline  
% Code-T5  & 220M (base) & ? & Enc-Dec  \\  %\hline  
% Incoder  & 1.3B/6.7B & ? & Dec-only \\ %\hline   
% CodeGen (Multi/Mono) & 350M/2B/6B/16B & 550k/650k & Dec-only \\ %\hline   
% % CodeGen-Multi  &  &  &  \\ %\hline   
% % CodeRL  &  &  &  \\ %\hline  
% % GPT  &  & ? &  \\ \bottomrule
% \end{tabular}
% }
% \end{center}
% \end{table}




%\subsection{Quantizing Code Generation Models}




\subsection{Weight Quantization}
Weight distributions have high variance with-in a kernel, accounting for outliers results in large quantization noise. This is particularly an issue with increasing matrix sizes in larger models. Figure~\ref{fig:pert-v-perr} shows how the quantization noise increases with model-sizes with per-tensor scales, but not with per-column scales. This reduced quantization noise with per-column scales explain why static (per-column) quantized models outperform static (per-tensor) quantized models.
\begin{figure}[h]
     \centering
         \includegraphics[width=0.8\linewidth]{figures/QuantizationNoisePerTvPerR.pdf}
         \caption{\textbf{\small{Weight quantization noise for CodeGen models across model sizes and granularity}}.}
         \label{fig:pert-v-perr}
\end{figure}
% Note that we can also reduce the quantization noise, by clipping the weight before rounding operations. Since weights are pre-determined the clipping values can be chosen before-hand based on the accuracy on validation data-set.
~\rayb{so what? Did we take any action based on this observation?}


\subsection{Activation Quantization}

The primary challenge in activation quantization is in choosing the quantization scales. With static-quantization, we will have to pick pre-determined scales based on validation data. This pre-determined scales is picked conservatively (i.e., we us large quantization ranges) to be large to avoid clipping when deployed. However, this would increase the quantization noise.

On the other-hand dynamic quantization allows us to adjust the scales for every input example and for every token, thereby making it attractive to reduce quantization noise. Dynamic quantization will be useful if we observe high variance in the max-values across different inputs/tokens. For example, ~\Cref{fig:dynamic} shows the max value of the activation across different layers in CodeGen-350M model.

%With static quantization, we will be picking a scale-value at 16 in layer 3 though most activation tensors will be $<2$, thereby effectively quantizing this layer with 4 bits instead of 8 as we only utilizing one-eight of the quantization range.% ~\rayb{why?}.


\begin{figure}[h]
     \centering
         \includegraphics[width=0.8\linewidth]{figures/ActivationDist.pdf}
         \caption{\textbf{\small Distributions of maximum activation value across different layers in CodeGen-350M model on validation data}.}
         \label{fig:dynamic}
\end{figure}

\subsection{Error Accumulation}

\sujan{I dont mind removing this subsection}

Quantization noise accumulates with depth, making deeper models more challenging to quantization. For example,~\Cref{fig:depth} shows the relative quantization noise with model depth for a CodeGen-6B model, showing quantization error growing with depth. 

On the other hand, a well trained network would have developed some robustness to small noise sources, which will help the activations from quantized networks match better with the unquantized network. This effect can be seen by observing error and correlation measured by comparing the activation of unquantized and quantized network, as shown in~\Cref{fig:depth} and~\Cref{fig:pearsons}, respectively. 


\begin{figure}[h]
     \centering
         \includegraphics[width=0.8\linewidth]{figures/ErrorAccumilations.pdf}
         \caption{\textbf{\small{Mean squared error per layer between activations from original model and quantized model. The error is estimated on a weight-only quantized CodeGen-6B model generating a token on HumanEval.}}}
         \label{fig:depth}
\end{figure}

%\subsection{Summary of key observations}
%Based on the analysis above, we summarize the key observation and insights as follows:
%\begin{itemize}
%    \item For quantizing weight of code generation model, 
%    \item For quantizing activation, 
%    \item 
%\end{itemize}



    

% \begin{figure}[h]
%      \centering
%          \includegraphics[width=0.4\textwidth]{figures/PearsonsCorr.pdf}
%          \caption{\small{\textbf{Pearson correlation per layer between activations from original model and quantized model. The correlation is estimated on a weight-only quantized CodeGen-6B model generating a token on HumanEval.}}}
%          \label{fig:pearsons}
% \end{figure}
    

% \begin{figure*}[t]
% \includegraphics[width=0.3\textwidth, height=0.2\textheight]{figures/placeholder-1.png}
% \centering
% \caption{Distribution of weight values in attention matrix and FFN. activation values}
% \label{fig:weight_distribution}
% \end{figure*}



%\section{Code-aware PTQ} \label{section:ptq}

%In this section, we present our proposed recipe for effectively performing code-aware PTQ on program synthesis models.


%\begin{figure}[t]
%\includegraphics[width=0.3\textwidth, height=0.2\textheight]{figures/cali_methods_p.jpeg}
%\centering
%\caption{Cutoff values with different C-PTQ calibration methods}
%\label{fig:cali_methods}
%\end{figure}


%\subsection{Language-aware/task-aware calibration}
%State-of-the-art program synthesis model are typically trained on code corpus that consists of multiple programming languages. For example, Incoder\cite{FriedD2022}, CodeRL\cite{LeH2022} supports code generation in $5$ languages, such as Python, Java and Javascript.

